ML-AQP: Query-Driven Approximate Query Processing based on Machine Learning

As more and more organizations rely on data-driven decision making, large-scale analytics become increasingly important. However, an analyst is often stuck waiting for an exact result. As such, organizations turn to Cloud providers that have infrastructure for efficiently analyzing large quantities of data. But, with increasing costs, organizations have to optimize their usage. Having a cheap alternative that provides speed and efficiency will go a long way. Concretely, we offer a solution that can provide approximate answers to aggregate queries, relying on Machine Learning (ML), which is able to work alongside Cloud systems. Our developed lightweight ML-led system can be stored on an analyst's local machine or deployed as a service to instantly answer analytic queries, having low response times and monetary/computational costs and energy footprint. To accomplish this we leverage the knowledge obtained by previously answered queries and build ML models that can estimate the result of new queries in an efficient and inexpensive manner. The capabilities of our system are demonstrated using extensive evaluation with both real and synthetic datasets/workloads and well known benchmarks.

==> evaluation_prev.tex <==
\section{Evaluation}
\subsection{Datasets \& Workloads}
For our evaluation we used both real and synthetic datasets along with synthetic workloads.

\textbf{Real} :
We used the \textbf{Crimes} dataset from \cite{crimesdata} and the \textbf{Sensors} dataset from \cite{sensors}. The Crimes dataset
holds $|\mathcal{R}_1| = 6.6\cdot{10^6} $ and the Sensors dataset $|\mathcal{R}_2| = 2.3 \cdot{10^6}$. We created \textbf{synthetic} workloads over these real datasets as real query workloads do not exist for this purpose as also instigated by \cite{wasay2017data}. For \textbf{Crimes} we generated predicates restricting the spatial dimension and for \textbf{Sensors} on the temporal dimension as essentially this is what the data analysts would be doing in an exploration task. For the predicates in the spatial dimension we used multiple multivariate-normal distributions to simulate the existence of multiple users. For the temporal dimension, we used a uniform distribution. We then recorded the results of a number of descriptive statistics (\texttt{COUNT}, \texttt{MEAN}, \texttt{SUM}, \texttt{MAX}) over different attributes in the datasets to sufficiently make sure the workload is randomized enough. 

\textbf{Synthetic}:
We also generated Synthetic datasets and workloads to stress test our implementation. Specifically, we generated datasets with varying dimensionality $[10, 20, 50, 100]$ to simulate data with large number of columns. Each column contains numbers generated from a uniform distribution $\mathcal{U}[10^{-8}, 10^{8}]$, therefore each point is $\mathbf{x} \in [10^{-8}, 10^{8}]^d$ where $d \in [10, 20, 50, 100]$. We then generated a number of query workloads with a varying number of selected columns to be restricted by predicates $p \in [2, 10, 20, 50]$ according to the dimensionality of each of the synthetic datasets. For instance, for a dataset with $d=10$ the resulting workloads were two, with the selected columns being $(2, 10)$. Each query point for those two datasets is then $\mathbf{q} \in [10^{-8}, 10^{8}]^{2p}$. The specification and the number of query workloads can be identified from Table \ref{tab:synth-workloads}.
\begin{table}
\caption{Synthetic Datasets and Workloads}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
& \multicolumn{4}{c|}{\textbf{Columns} ($d$)} \\ \hline
\textbf{Predicates }($p$) & $10$ & $20$ & $50$ & $100$ \\ \hline
$2$ & \checkmark & \checkmark  & \checkmark & \checkmark \\ \hline
$10$ & \checkmark & \checkmark  & \checkmark & \checkmark \\ \hline
$20$ &  & \checkmark  & \checkmark & \checkmark \\ \hline
$50$ &  &   & \checkmark & \checkmark \\ \hline
\end{tabular}
\label{tab:synth-workloads}
\end{table}

We also describe the query generation process in Algorithm \ref{alg:query-gen}. We first set the number of queries $N$ and number of predicates and columns in our datasets $\mathcal{D}$, $\mathcal{P}$. The retrieved range size $r$ is obtained by first finding the bin width and height (=frequency) of a histogram over the columns. This is to ensure similar selectivities among the different queries. We then loop through over the parameters issued and generated queries using the provided algorithms. Where the $random$ function returns a random vector of size $p$ over the given range, and $randomBit$ generates a random bitmask for the selection of columns taking part in the query. Then the lower-bound and upper-bound for the given predicates is set and we execute the query over the restricted space given by the bounds over the selected columns by $b$ using dataset $d$.

\begin{algorithm}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
 \caption{Generating Queries}
 \label{alg:query-gen}
 \Input{$N$, number of queries}
 \Input{$\mathcal{D} = [10, 20, 50, 100]$, number of columns in datasets}
 \Input{$\mathcal{P}= [2, 10, 20, 50]$, number of predicates (selected columns)}
 \Input{$r$, range size retrieved from histogram to ensure similar selectivities}
 \For {$d\in \mathcal{D}$}{
 	\For {$p \in \mathcal{P}$}{
    	\For {$i= 1 \textbf{ to } N$}{
        	$\mathbf{z} \gets random([10^{-8}, 10^8], p)$ \;
            $\mathbf{b} \gets randomBit([0, d], p)$ \; 
            $\mathbf{lb} \gets \mathbf{z}-\frac{r}{2}$ \;
            $\mathbf{ub} \gets \mathbf{z}+\frac{r}{2}$ \;
            $\mathbf{q}_i^{(m)} \gets [\mathbf{lb}, \mathbf{ub}]$\;
            $y_i \gets executeAggregates(\mathbf{q}_i^{(m)}, d)$ \;
            $\mathbf{q}_i \gets (\mathbf{q}_i^{(m)},y)$ \;
            $\mathcal{W}_{d,p} \cup \{\mathbf{q}_i\}$\;
        }
    }
 }
 \Output{Resulting workloads $\mathbf{W} = (\mathcal{W}_{10,2}, \ldots, \mathcal{W}_{d,p}), \forall d\in \mathcal{D}, \forall p\in \mathcal{P}$}
\end{algorithm}

\subsection{Implementation \& Experimental Environment}
To implement our algorithms we used \texttt{scikit-learn} , \texttt{XGBoost}\cite{chen2016xgboost} and an implementation of the \texttt{Growing-Networks} algorithm \cite{marsland2002self,growingnetworks}. We performed our experiments on a desktop machine with a Intel(R) Core(TM) i7-6700 CPU @ 3.40GHz and 16GB RAM. The GrowingNetworks and algorithm was used for clustering mainly because of its invariance to selecting a pre-defined number of clusters and it's ability to naturally grow (as required by our adaptability mechanisms). XGBoost was used as the supervised learning algorithm because of its superior accuracy to other algorithms we tested and shown as part of our evaluation.

\subsection{Accuracy}
\begin{figure*}[!htbp]
\begin{center}
\begin{tabular}{ccc}
\includegraphics[height=4cm,width=4.5cm,keepaspectratio]{rel-errorVSpredicates}
\includegraphics[height=4cm,width=4.5cm,keepaspectratio]{rel-errorVScolumns}
\includegraphics[height=4cm,width=4.5cm,keepaspectratio]{rel-errorVSqueries}\\
\end{tabular}
\caption{Evaluating accuracy across statistics at different conditions using : (from left to right) increasing number of predicates, columns and queries}
\label{fig:acc-vs-conditions}
\end{center}
\end{figure*}

We measured the accuracy of our implementation using both \textit{synthetic} and \textit{real} datasets. Overall, we report that our system is able to give good enough estimations that will keep on getting better as more queries are being processed. All of the figures report the \textit{Relative Error} and unless stated otherwise, corresponds to the \textit{median} relative error over a number of iterations.

We first examine the \textit{predictability} of different descriptive statistics operators using a variety of supervised learning models. The experiments were conducted using our Synthetic workloads to test accuracy across different number of columns and predicates. The reported quantities are the median relative errors across all workloads with the standard deviation for each statistic. Where, \texttt{Ridge} is a Regularized Linear Regression model, \texttt{SGD} is a linear regression model trained on-line using SGD, \texttt{SVR} is a Support Vector Regression model with an \textit{rbf} kernel, \texttt{XGB} is the XGBoost model, and \texttt{NN} is a Multi-Layer Perceptron Network. None of the models was hyper-tuned to provide the purest accuracy as we wanted to test whether different statistics could be estimated by different models, thus indicating the need to choose optimal models at training time. Figure \ref{fig:accuracy-aggsXmodels} shows the results of this experiment. First of all, it's clear that SGD and NN have not \textit{converged} as the number of queries might not sufficient\footnote{1000 queries were used} and such are algorithms are known for their need of many training examples. Our second takeaway, is that for \texttt{COUNT} we get the highest error with relatively high variation across the different workloads. This is not to say that \texttt{COUNT} would always be un-predictable as for some real datasets it could very well be the case that \texttt{COUNT} is highly predictable. What's more important here is that all of the statistics can be adequately predicted by a single algorithm, that being \texttt{XGB}. Which is an advantage to us, as the system can be optimized for storing such models and can be designed around this single class of model instead of trying to accommodate a variety of them, each with its own limitations and restrictions.

\begin{figure}[htbp]
\begin{center}
\includegraphics[height=4cm,width=6cm]{TEMP.eps}%rel-error-modelsXaggregates
\caption{Relative Error across different models and statistics}
\label{fig:accuracy-aggsXmodels}
\end{center}
\end{figure}

Using the best model out of the previous experiment (\texttt{XGB}), we evaluated accuracy of in predicting the different statistics under different conditions, shown in Figure \ref{fig:acc-vs-conditions}. As expected, the increase in number of predicates used and number of columns has a negative impact on accuracy. The increase in error is no more than linear w.r.t to increasing the number of predicates and columns. With statistics such as \texttt{MEAN}, \texttt{SUM}, \texttt{MAX} being less impacted by this change, as their error seems to be invariant towards the beginning. In addition, still as expected, the error decreases with an increasing number of queries being used for training, with the error reaching a plateau after about $300$ queries.

In our analysis we have also used real datasets to demonstrate the applicability of our system under real conditions. As evident from Figure \ref{fig:accuracy-aggsXdata} our system is able to provide estimations for different descriptive statistics across different types of real-datasets with relative error below $12\%$. A difference of more than $10\%$ between the two datasets is also clear with that being attributed to the extra predicate placed on the Crimes workloads. As, Crimes are restricted spatially by two dimensions and Sensors temporally by one. We see the effects that the dimensionality and number of predicates in following experiments. In addition, Figure \ref{fig:acc-vs-queries} shows how accuracy is increased as the number of queries used for training is increased. Around $10^4$ queries are needed to reach minimum relative error for Crimes, at which point no more accuracy is gained by processing more queries. On the other hand, Sensors need just a bit less than $5\cdot 10^4$ to accurately learn estimating descriptive statistics thus backing up our claim for Sensors being a much easier distribution to learn. 

\begin{figure}[!htbp]
\begin{center}
\includegraphics[height=4cm,width=6cm,keepaspectratio]{crimes-sensors-rel-error}
\caption{Relative error for different descriptive statistics across two real datasets}
\label{fig:accuracy-aggsXdata}
\end{center}
\end{figure}

\begin{figure}[!htbp]
\begin{center}
\begin{tabular}{cc}
\includegraphics[height=4cm,width=4.5cm,keepaspectratio]{TEMP-TEMP}%accuracy-vs-_queries-crimes
\includegraphics[height=4cm,width=4.5cm,keepaspectratio]{accuracy-vs-_queries-sensors}\\
\end{tabular}
\caption{Accuracy over number of queries:(Left) Crimes (Right) Sensors}
\label{fig:acc-vs-queries}
\end{center}
\end{figure}
\textcolor{blue}{accuracy experiment with varying number of clusters}
% \begin{figure*}[!htbp]
% \begin{center}
% \includegraphics[height=3.5cm,width=8.5cm]{s-aqp-vs-ml-aqp}
% \caption{}
% \label{fig:accuracy-aqpvsml}
% \end{center}
% \end{figure*}
\subsection{Accuracy over alternative representations}
We investigate the possibility that our representation is not optimal. It could be more wise to build separate models for queries with predicates in specific columns. This way the dimensionality of the query vector $\mathbf{q}^{(m)}$ is reduced from $\mathbf{m} \in \mathbb{R}^{2d}$ to $\mathbf{m} \in \mathbb{R}^{2p}$ with $p\leq d$ always. Although this might increase accuracy, we note that it decreases flexibility as we can no longer consider all queries for a certain schema but we need to add another layer of grouping w.r.t to the columns being asked in the predicates.

\begin{figure}[!h]
\begin{center}
\begin{tabular}{cc}
\includegraphics[height=4cm,width=4.5cm,keepaspectratio]{Length_of_vector__predicates-across-models}
\includegraphics[height=5cm,width=4.5cm,keepaspectratio]{Length_of_vector__columns-across-models}\\
\end{tabular}
\caption{Accuracy across different representations (Left) Length of query vector $\mathbf{m}\in \mathbb{R}^{2p}$ (Right) Length of query vector $\mathbf{m}\in \mathbb{R}^{2d}$}
\label{fig:acc-repre}
\end{center}
\end{figure}
However, consulting Figure \ref{fig:acc-repre}, we see that our assumption does not hold, as the accuracy does not increase with this different representation. On the contrary, we see a decrease in accuracy along with an increase in standard deviation across all aggregates.

\subsection{Accuracy of error estimation}
Error estimation is an integral part of our system. Its importance is paramount for the detection of concept drift. Our method described in Section \ref{sec:detect} and Eq. \ref{eq:error} provide a simple yet effective way of mitigating such circumstances. When estimating the error it is important to note that there is no need to correctly estimate the true errors as long as the estimated errors have a strong positive correlation with the true error. Minimizing the loss between the true error and the estimated error is not our objective in this case. Instead, we wish our estimations to be correlated such that whenever the true error decreases or increases with respect to a given query the estimated errors should do the same. So it the magnitude of the estimations and their difference  with the actual errors do not matter. 
\subsection{Performance \& Storage}
Next, we evaluate the performance and storage requirements of our system. As the designed system is invariant to the selection of supervised models we check the performance of a number of models as we did with the accuracy experiments. Mainly because, we would like to identify the most efficient models when training and when predicting. We used a synthetic workload with $p=50$ and $d=100$ to obtain an upper-bound on the performance across models. For \textit{Prediction Time}, as seen in Figure \ref{fig:perf}(left), we record the average prediction time along with the standard deviation for each model. As expected, \texttt{SVR} has the worst performance as it has to evaluate a summation of the kernel distance between the support vectors and the training vector. However, please note that all times are less than a millisecond, guaranteeing efficient statistic estimation no matter the model used. Even though there are a number of models trained as explained in Section \ref{sec:query-answer}, the complexity associated  with going through the models is $\mathcal{O}(k)$ with $k$ usually being small. Thus the bottleneck being the evaluation of the model itself to provide an estimation. It is also important to consider that this is essentially all the cost carried by our system as it will reside on the user's local machine and often in memory, thus relieving any latency and monetary costs for using the cloud. As for training the individual models, we vary the number of tuples/training samples and examine the time required by the different models. For \texttt{SVR} we stop measuring after $1.6\cdot 10^4$ training samples as solving the dual problem posed by the algorithm is no longer efficient and should not be used. As expected, the performance of all models begin to deteriorate as a there are a number of optimizations going on when trying to minimize the objective function given to them. Although \texttt{XGB} appears to perform the worst, for an increasing number of tuples, we note that the time required is no more than $25$ seconds. This is far better better than any other deep learning model which might require a large amount of resources and time to train, consequently translating to a huge bill for small-scale organizations.
\begin{figure}[!h]
\begin{center}
\begin{tabular}{cc}
\includegraphics[height=4cm,width=4.5cm,keepaspectratio]{perf-ave-pred-time}
\includegraphics[height=5cm,width=4cm,keepaspectratio]{perf-training}\\
\end{tabular}
\caption{Performance across different models (Left) Average Prediction time (Right) Training time across models with an increasing number of tuples.}
\label{fig:perf}
\end{center}
\end{figure}

Examining Figure \ref{fig:storage} we see the storage requirements across different models to be used. The size is in \textit{kilobytes} which translates to a negligent cost fulfilling one of our initial requirements stating that we need something light-weight to reside in memory and be at the immediate disposal of a user. The exhibited results are for one individual model therefore the resulting storage cost is $k$ times the initial one. This can prove to be a preventive cost, especially for \texttt{SVR} as becomes $k \gg 1000$. Thus it is preferable to use some other model in such cases.

\begin{figure}[!htbp]
\begin{center}
\includegraphics[height=4cm,width=6cm]{per-stor}
\caption{Storage requirements for different models}
\label{fig:storage}
\end{center}
\end{figure}

==> future.tex <==
\section{Future Work \& Limitations}
%More advaned models and techniques to increase accuracy
%NLP to do automatic feature extraction
%Data Updates 

==> supervised_learning.tex <==
\section{Local Model Estimation}
\label{sec:query-answer}
\subsection{Local Supervised Model}
%Data is partitioned - We can use each partition to train separate models - What's the task, minimizing squared error loss, multitude of ML algorithms that can do that following different techniques. Result is an ML model which can in turn be transmitted to the user's/analysts local machine. A number of models can be trained and transmitted w.r.t the query parameters the user has issued so far, and the kind of aggregates. For each aggregate we train different model. The analyst uses the ML models to avoid executing queries in the cloud - Gets back estimated results along with an estimation of the error.(Figure, x - parameter, y- result, shade error, different color lines aggregates). Error is the predicted generalization error given by the algorithm can be used to construct error bounds.
Each query answer $y$ form the pair $(\mathbf{q},y) \in \mathcal{C}_{t}$ is estimated through an unknown function $g(\cdot)$. Such function produces query-answers w.r.t an unknown conditional distribution $P(y|\mathbf{q})$. 
Our aim is to approximate the \textit{true} functions 
$g$ for each aggregate functions (descriptive statistics) e.g., count, average, min, max, sum, etc. Supervised ML algorithms are adopted, to minimize the expected prediction loss between the actual query-answer $y = g(\mathbf{q})$ from the true function $g(\cdot)$ and a predicted $\hat{y}$ from an approximated function $\hat{f}(\cdot)$ generated by the model: 
\begin{equation}
\label{eq:obj-error}
\min \mathbb{E}_{\mathbf{q}}[\mathcal{L}(g(\mathbf{q}), \hat{f}(\mathbf{q}))]
\end{equation}
The loss $\mathcal{L}(\cdot, \cdot)$ can be measured using \textit{absolute} or \textit{squared} loss functions :
\begin{eqnarray}
\mathcal{L} = |g(\mathbf{q}) - \hat{f}(\mathbf{q})| \mbox{ or } \mathcal{L} = (g(\mathbf{q}) - \hat{f}(\mathbf{q}))^2.
\end{eqnarray}
Supervised learning algorithms minimize such expected prediction loss using \textit{training} examples, which they use to learn the true function $g$. Such training examples are the
query-answer pairs in $\mathcal{C}_{t}$, which are drawn from $P(y|\mathbf{q})$. Hence, by minimizing 
the \textit{sample} error we expect to obtain good 
estimation over any unseen query $\mathbf{q}$. The objective in \textit{Eq.}\ref{eq:obj-error} is to minimize the Mean Squared Error (MSE): 
\begin{equation}
\frac{1}{t}\sum_{\tau=1}^t(y_{\tau} - \hat{f}(\mathbf{q}_{\tau}))^2.
\label{eq:objective}
\end{equation}
Note, various supervised learning algorithms minimize a variant of the objective in (\ref{eq:objective}) including a regularization parameter as a technique to avoid \textit{overfitting} \cite{friedman2001elements}.

After having partitioned the query space into disjoint 
clusters $C_1,\ldots, C_K$, we therein train $K$ 
different supervised learning models, $\mathcal{M}=\{\hat{f}_1,\ldots, \hat{f}_K\}$ that 
associate query vectors $\mathbf{q}$ belonging to cluster $C_{k} \in \mathcal{C}$ with their corresponding response outputs $y$.
That is, each \textit{local} model $\hat{f}_{k}$ is trained using the query-response pairs $(\mathbf{q},y) \in \mathcal{C}_{t}$ from those queries $\mathbf{q}$ which belong to $C_{k} \subset \mathcal{C}_{t}$ such that $\mathbf{w}_{k}$ is the closest cluster head of those queries.
%%Example below can be omitted
Another advantage of partitioning the 
query vectorial space and obtaining multiple 
statistical models is that we obtain lower estimation error across the query space. 
As the query space is now partitioned and different models are fitted across different partitions, we end up with an estimation of the \textit{generalization} error, which is different w.r.t to a given model. To visualize this statement, Figure \ref{fig:err-bands} is constructed in 2D for clarity. 
Two different actual functions $g_{1}(\mathbf{q})$ and $g_{2}(\mathbf{q})$ are approximated using the estimate functions $\hat{f}_{1}$ and $\hat{f}_{2}$ plotted in red and blue. These represent different aggregates of the response variable $y$. Based on the query space partitioning, for each sub-space a different model is trained and a different estimation of the generalization error is obtained by the respective algorithm. Hence, the analyst is now aware which results they can trust more and for which query parameter-values the result is hard to estimate (i.e., it has more variability). As seen from the example, the analyst should trust the results for $\hat{f}_{2}$ with a grain of salt because of the wider error bounds across part of the domain. Not using the clustering process would translate to a single uniform generalization error across the complete parameter space which is often an under-statement of the true error.

\begin{figure}
\begin{center}
\includegraphics[height=4cm,width=6cm]{examples-error-bands}
\caption{The approximated true function for two different aggregates, along with different error bands; x-axis is the query parameter(s) and y-axis is the response variable $y$}
\label{fig:err-bands}
\end{center}
\end{figure}

\subsection{Query Results Prediction}
%How are estimations obtained. Show that the strategy is an ensemble learning strategy in which the voting mechanism supported is that the closer learner has full voting rights. \sum_ all learners*weight where weight is 1 if closest and weight is 0 otherwise
Once the \textit{training} process is complete for all the models $\hat{f}_{k}$ over their query clusters $C_{k}$, $k \in [K]$, 
the models are transmitted to the analysts and 
are used for predicting query answers for any subsequent unseen query. 
This partition-and-local-learning methodology effectively 
assumes an \textit{ensemble} learning strategy for our system. By adopting such an ensemble learning strategy, the various models have \textit{voting rights}, meaning that each one of them contributes to the final query answer prediction for a given query by casting a vote. However, our strategy is to revoke voting rights for models, which do not represent 
the query sub-space space that a given query belongs to. 
Hence, an \textit{authoritative} power over the rest of the models is assigned to the most representative model thus returning to the user a prediction from the most appropriate model. Empirically, this was shown to work better than alternative strategies, most likely because considering the prediction contribution of other models, introduces noise into our final prediction. Formally, the proposed ensemble prediction is:

\begin{eqnarray}
& \hat{y} = \sum_{k=1}^{K}\mathcal{I}_{k}\hat{f}_{k}(\mathbf{q})  \\
\text{with} & \mathcal{I}_{k} = \begin{cases}
1 \quad \text{if} \quad \mathbf{w}_{k} = \arg\min_{i \in [K]}\lVert \mathbf{q}-\mathbf{w}_{i}\rVert \\
0 \quad \text{otherwise} \quad 
\end{cases}  \nonumber 
\end{eqnarray}
The indicator function $\mathcal{I}$ returns zero if the $k$-th representative cluster-head with does not match the closest representative to the incoming query $\mathbf{q}$.

\subsection{Error Estimation}
\textit{Prediction Intervals}

==> user_profiling.tex <==
\section{Query Patterns Clustering}
%Parameter values issued by different users often form clusters (SDSS graph) ref.
%Users are potentially interested in vastly different regions of the dataset thus issuing queries with different parameter values
%Clustering is a machine learning method that allows for this grouping of similar parameter values into disjoint sets. This would allow for more accuracy in the models trained subsequently and more would allow for the transmission of more approriate models to user's who have executed queries similar to those belonging to the clsuter associated with the model.
%Explain the Process of clustering. Having a log filled with queries and their different parameters. We hold their meta-vectors.
%Clustering is then, and give the objective function for clustering algorithms. Can use any kind of off-the-shelf and thoroughly tested clustering algorithms (references). Clustering results in a number of cluster-heads (either pre-defined or given by the algorithm). Each cluster-head has a number of queries associated with it. Figure for clustering showing Voronoi cells
%Then every query is associated with a cluster. Thus we end up with k disjoint sets. Those k disjoint sets are then used to train Supervised Machine Learning algorithms that can predict the results of new queries.
Analysts extract information over large datasets by issuing a number of queries restricting the data-space and returning descriptive statistics. It is a common event that the patterns of different analysts will be the same. Figure \ref{fig:clusters} shows the formation of clusters for two different query parameters from a real query workload obtained from Sloan Digital Sky Survey (SDSS)\cite{szalay2002sdss}. 
It is shown that the queries form clusters around certain parameter values depicting the interests of those particular analysts over the underlying data sub-spaces. In light of this we follow an approach to group together queries with similar parameter values using clustering techniques.

\begin{figure}
\begin{center}
\includegraphics[height=4cm,width=4cm]{clusters-queries}
\caption{Parameters forming clusters in a real workload (Source SDSS \cite{szalay2002sdss})}
\label{fig:clusters}
\end{center}
\end{figure}
Clustering is an unsupervised ML technique that allows for the discovery of said clusters within a vectorial (real-valued) space. The result of this method is to produce a number of groups that partition the issued queries into disjoint subsets of similar queries. Partitioning is fundamental to get more accurate ML models for predictive analytics. Having a number of different statistical models learn different sub-sets of data is proven to work 
more efficiently in terms of \textit{explainability/model-fitting} and \textit{predictability} than having one unique global model learn everything. This methodology of learning/training different models over different data subspaces reduces variance in both the \textit{predictors} and our \textit{response} variable as shown on Table \ref{tab:variance}. Such methodology is referred to as \textit{ensemble learning}\cite{friedman2001elements} and is widely used in predictive modeling. 
%Reference to ED architecture
% Therefore, the models transmitted to the analyst's local machine from the ED are only the ones that were trained with subsets of queries that included the user's issued queries to that ED. Hence, such models \textit{capture} the exploratory interests of the ED's analysts analyzing the data subspaces by issuing analytics queries. 

\begin{table}
\caption{\textcolor{blue}{show correlation or mutual information instead of reduction in parameter and response variance}
}
\begin{tabular}{|c|c|c|} 
 \hline
 & \textbf{Global Model $\mathcal{M}$} & \textbf{Local Models $\mathcal{M}_{k}$} \\ \hline
 \textbf{Variance $\mathbf{m}$} & $0.124$ &  $0.0017$ \\ \hline
 \textbf{Variance $y$} & $1.5\cdot10^{10}$ & $3.5\cdot10^8$ \\ \hline
\end{tabular}
\label{tab:variance}
\end{table}

Consider a discrete time domain $t \in \mathbb{T} = \{1, 2, 3, \ldots\}$, where at each time instance $t$ an analyst issues a query which is translated to a meta-vector $\mathbf{q}_{t}$. The query is executed and an answer is produced $y_{t}$, thus, forming the query-answer pair $(\mathbf{q}_{t},y_{t}), t \in \mathbb{T}$. The issued queries are stored in a growing set of pairs $\mathcal{C}_{t} = \{(\mathbf{q}_1, y_1),\ldots, (\mathbf{q}_t, y_t)\} = \mathcal{C}_{t-1} \cup \{(\mathbf{q}_{t},y_{t})\}$. 

Given this growing set, we wish to incrementally extract significant knowledge from the query vectors to approximate the data subspaces on interest and then sequentially develop \textit{local} ML models that efficiently  predict the associated outputs given unseen queries. 
Such knowledge extraction is achieved by on-line partitioning the query vectors $\{\mathbf{q}_{1}, \ldots, \mathbf{q}_{t}\}$ from the set $\mathcal{C}_{t}$ into disjoint clusters that represent the query patterns of the  analysts. 
Fundamentally, within each cluster the queries are much more \textit{similar} than the queries in other clusters. 
In our case, query similarity quantifies how close the parameter values (across different queries) are to each other in a parameter space. That is, similar queries $\mathbf{q}$ and $\mathbf{q}'$ are grouped together into $K$ clusters with query similarity being the Euclidean distance in a real-valued vectorial space: $\lVert \mathbf{q} - \mathbf{q}' \rVert$.
The main objective of a query clustering algorithm is then to minimize the \textit{distance} of all queries to a corresponding cluster \textit{representative}, which is essentially a \textit{pseudo}-query representing the analysts query patterns and best represents each cluster; it is often the \textit{mean}-vector of all queries associated with that cluster.
The $K$ query representatives $\mathcal{W} = \{\mathbf{w}_{1}, \ldots, \mathbf{w}_{K}\}$ are estimated to optimally represent the queries in $\mathcal{C}_{t}$ such that they incrementally minimize the expected quantization error:
\begin{equation}
\mathbb{E}[\min_{k}\lVert \mathbf{q}-\mathbf{w}_{k} \rVert^{2}].
\end{equation}
Each query $\mathbf{q}$ becomes associated with the closest 
representative: 
\begin{equation}
\label{eq:closest}
\mathbf{w}^{*} = \arg\min_{\mathbf{w} \in \mathcal{W}}\lVert \mathbf{q}-\mathbf{w}\rVert
\end{equation}
Based on this partition of the query space defined by the queries in $\mathcal{C}_{t}$, we then produce $K$ query-disjoint sub-sets $\mathcal{C}_{t}= \mathcal{C}_1\ \cup \ldots \mathcal{C}_K$, such that $\mathcal{C}_k\cap\mathcal{C}_l \equiv \emptyset$ for $k\neq l$ and $\mathcal{C}_{k} =\{(\mathbf{q},y) \in \mathcal{C}_{t} | \mathbf{w}_{k} = \arg\min_{\mathbf{w} \in \mathcal{W}}\lVert \mathbf{q}-\mathbf{w}\rVert^{2}\}$. A local predictive ML model can now be trained over each query-disjoint subset of query-answer pairs $\mathcal{C}_{k}, k \in [K]$.
